LiveFC: A System for Live Fact-Checking of Audio Streams

The advances in the digital era have led to rapid dissemination of information. This has also aggravated the spread of misinformation and disinformation. This has potentially serious consequences, such as civil unrest. While fact-checking aims to combat this, manual fact-checking is cumbersome and not scalable. While automated fact-checking approaches exist, they do not operate in real-time and do not always account for spread of misinformation through different modalities. This is particularly important as proactive fact-checking on live streams in real-time can help people be informed of false narratives and prevent catastrophic consequences that may cause civil unrest. This is particularly relevant with the rapid dissemination of information through video on social media platforms or other streams like political rallies and debates. Hence, in this work we develop a platform named LiveFC, that can aid in fact-checking live audio streams in real-time. LiveFC has a user-friendly interface that displays the claims detected along with their veracity and evidence for live streams with associated speakers for claims from respective segments. The app can be accessed at http://livefc.factiverse.ai and a screen recording of the demo can be found at https://bit.ly/3WVAoIw.

==> claim_stats.tex <==


\begin{tikzpicture}
\edef\mylst{"169","147"}
\edef\explora{"170","205"}

    \begin{axis}[
            ybar=5pt,
            width=1\textwidth,
            bar width=0.05,
            every axis plot/.append style={fill},
            grid=major,
            xtick={1, 2},
            xticklabels={Biden, Trump},
            xlabel={},
            ylabel style = {font=\tiny},
        yticklabel style = {font=\boldmath \tiny,xshift=0.12ex},
        xticklabel style ={font=\tiny,yshift=0.5ex},
            ylabel={Number of claims},
            enlarge x limits=0.20,
            ymin=0,
            ymax=300,
            legend style ={font=\tiny},
            area legend,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend entries={SUPPORTED, DISPUTED},
            legend cell align={left},
            legend pos=north west,
            legend columns=-1,
            legend style={/tikz/every even column/.append style={column sep=0.2cm}},
        ]
        \addplot+[
            ybar,
            plotColor2*,
            draw=black,
            postaction={
                    pattern=north east lines
                },
        ] plot coordinates {
                (1,169)
                (2,147)

            };
        \addplot+[
            ybar,
            plotColor1*,
            draw=black,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
    nodes near coords align={vertical},
            postaction={
                    pattern=north west lines
                },
        ] plot coordinates {
                (1,170)
                (2,205)

            };
 

    \end{axis}


    
\end{tikzpicture}


==> exemplars-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: A cat chases a rat 6 hours after the rat runs. cat takes 4 hours to reach the rat. If the average speed of the cat is 90 kmph, what s the average speed of the rat?
\\ & \textbf{Options}: ['A)32kmph', 'B)26kmph', 'C)35kmph', 'D)36kmph', 'E)32kmph']
\\ & \textbf{Rationale:} Cat take 10 hours and rat take 4 hours...then Distance is 90*4.so speed of rat is (90*4)/10 = 36kmph 
\textbf{Answer: D}
 \\\cline{2-2}
 & \textbf{Question:}  A business executive and his client are charging their dinner tab on the executive's expense account.The \dots?
 \\ & \textbf{Options}: ['A)69.55\$', 'B)50.63\$', 'C)60.95\$', 'D)52.15\$', 'E)53.15'] \\
 & \textbf{Rationale}:  let x is the cost of the food
1.07x is the gross bill after including sales tax
1.15* 1.07x=75 \textbf{Answer}: C \\\cline{2-2}
 & \textbf{Question:}John and David were each given X dollars in advance for each day they were expected to perform at a community festival. John eventually,\dots? 
 \\ &\textbf{Options}: 'A)11Y', 'B)15Y', 'C)13Y', 'D)10Y', 'E)5Y' \textbf{Rationale:} \dots  \textbf{Answer:} A\\\cline{2-2}
  & \textbf{Question:}A contractor undertakes to do a piece of work in 40 days. He engages 100 men at the beginning and 100 more after 35 days and completes the work in stipulated time. If he had not engaged the additional men, how many days behind schedule would it be finished?? \\
 & \textbf{Options}: 'A)2', 'B)5', 'C)6', 'D)8', 'E)9'
  \textbf{Rationale:}  [(100$\times$ 35)+(200$\times$ 5)] men can finish the work in 1 day
therefore 4500 men can finish the work in 1 day. 100 men can finish it in  $\frac{4500}{100}$ = 45 days.
This is 5 days behind Schedule 
  \textbf{Answer:} A\\\cline{2-2}
    & \textbf{Question:} A can do a job in 9 days and B can do it in 27 days. A and B working together will finish twice the amount of work in ------- days? \\
 & \textbf{Options}: 'A)22 days', 'B)18 days', 'C)22 6/2 days', 'D)27 days', 'E)9 days'
  \textbf{Rationale:} 1/9 + 1/27= 3/27 = 1/9
9/1 = 9*2 =18 day
  \textbf{Answer:} B\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The average age of three boys is 15 years and their ages are in proportion 3:5:7. What is the age in years of the youngest boy?
\\ \colorg & \colorg \textbf{Options}: ['A)9', 'B)10', 'C)11', 'D)12', 'E)13']
\\\colorg & \colorg\textbf{Rationale:}3x + 5x + 7x = 45,
x =3,
3x = 9
\textbf{Answer: A}
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Can you deduce the pattern and find the next number in the series? $6, 14, 26, 98$?

  \textbf{Options}: [''A)276', 'B)277', 'C)278', 'D)279', 'E)None of these']] \\\colorg
 & \colorg\textbf{Rationale}:  $6 = 1^1 + 2^1 + 3^1, 
14 = 1^2 + 2^2 + 3^2,
36 = 1^3 + 2^3 + 3^3,
98 = 1^4 + 2^4 + 3^4$
Thus the next number 
 \textbf{Answer}: A \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}In covering a distance of 42 km, A takes 2 hours more than B. If A doubles his speed, then he would take 1 hour less than B. A's speed is:? 
\\ \colorg & \colorg \textbf{Options}: 'A)5 km/h', 'B)7 km/h', 'C)10 km/h', 'D)15 km/h', 'E)25 km/h' \textbf{Rationale:} Let A's speed be X km/hr.
Then, 42/x - 42/2x = 3
6x = 42
x = 7 km/hr \textbf{Answer:} B\\\cline{2-2}\colorg
  &\colorg \textbf{Question:}Find  the number which when multiplied by 15 is increased by 196. \\\colorg
 &\colorg \textbf{Options}: 'A)14', 'B)20', 'C)26', 'D)28', 'E)30'
  \textbf{Rationale:}  Solution
Let the number be x .
Then, 15x - x = 196
‹=›14x = 196
x ‹=› 14 
  \textbf{Answer:} A\\\cline{2-2}\colorg
    & \colorg\textbf{Question:} A certain sum of money at simple interest amounted Rs.980 in 3 years at 5\% per annum, find the sum? \\\colorg
 & \colorg\textbf{Options}: 'A)867', 'B)855', 'C)299', 'D)852', 'E)903'
  \textbf{Rationale:} 980 = P [1 + (3*5)/100]
P = 852 
  \textbf{Answer:} D\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\aqua{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_aquarat}
%\vspace{-0.25cm}
\end{table*}





















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | increase ( decrease ) |
average yield | 2.75\% ( 2.75 \% ) |
volume | 0.0 to 0.25 |
energy services | 2013 |
fuel recovery fees | 0.25 |
recycling processing and commodity sales | 0.25 to 0.5 |
acquisitions / divestitures net | 1.0 |
total change | 4.25 to 4.75\% ( 4.75 \% ) |
\\ & \textbf{Question}: what is the ratio of the acquisitions / divestitures net to the fuel recovery fees as part of the expected 2019 revenue to increase
\\ & \textbf{Rationale:} ans=( 1.0 / 0.25 )
\textbf{Answer: }  The answer is 4
 \\\cline{2-2}
 & \textbf{Table:}  ( in millions ) | 2009 | 2008 | 2007 |
sales and transfers of oil and gas produced net of production andadministrative costs |  -4876 ( 4876 ) |  -6863 ( 6863 ) |  -4613 ( 4613 ) |
\dots
 \\ & \textbf{Question}: were total revisions of estimates greater than accretion of discounts?
\\
 & \textbf{Rationale}: \dots   \textbf{Answer}: The answer is yes  \\\cline{2-2}
 & \textbf{Table:} | 2007 | 2008 | change |
capital gain distributions received | 22.1 |  5.6 | -16.5 ( 16.5 ) |
other than temporary impairments recognized | -.3 ( .3 ) | -91.3 ( 91.3 ) | -91.0 ( 91.0 ) |
net gains ( losses ) realized onfund dispositions | 5.5 | -4.5 ( 4.5 ) | -10.0 ( 10.0 ) |
net gain ( loss ) \dots
 \\ &\textbf{Question}: what percentage of tangible book value is made up of cash and cash equivalents and mutual fund investment holdings at december 31 , 2009?
\textbf{Rationale:} ( 1.4 / 2.2 )  \textbf{Answer:}  The answer is 64\%\\\cline{2-2}
  & \textbf{Table:} in millions | 2009 | 2008 | 2007 |
sales | 5680 | 6810 | 6530 |
operating profit | 1091 | 474 | 839 |
\\
 & \textbf{Question}: north american printing papers net sales where what percent of total printing paper sales in 2009?
   \textbf{Rationale:} x0=( 2.8 * 1000 ), ans=( x0 * 5680 )
  \textbf{Answer:} The answer is 49\%\\\cline{2-2}
    & \textbf{Table:}  in millions | december 312015 | december 312014 |
total consumer lending | 1917 | 2041 |
total commercial lending | 434 | 542 |
total tdrs | 2351 | 2583 |
nonperforming | 1119 | 1370 |
\dots
 \\
 & \textbf{Question}: what was the change in specific reserves in alll between december 31 , 2015 and december 31 , 2014 in billions?
  \textbf{Rationale:} ( .3 - .4 )
  \textbf{Answer:}  The answer is -0.1\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | 2008 | 2007 |
balance at beginning of year | 23.2 | 56.4 |
additions due to acquisition of allied | 582.9 | 2014 |
additions based on tax positions related to current year | 10.6 | 16.3 |
reductions for tax positions related to the current year | -5.1 ( 5.1 ) | -17.2 ( 17.2 ) |
\dots
\\ \colorg & \colorg \textbf{Question}: in 2008 what was the change in the gross unrecognized tax benefits in millions
\\\colorg & \colorg\textbf{Rationale:}  (611.9 - 23.2 )
\textbf{Answer: } The answer is 588.7
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} december 31 2004 | 1054 |
december 31 2005 | 1216 |
december 31 2006 | 1219 |
december 31 2007 | 2566 |
  \textbf{Question}: what was devon's average translation adjustments included in accumulated other comprehensive income ( in millions ) from 2004 through 2007?
\textbf{Rationale}: x0=( 1054 + 1216 ), x1=( x0 + 1219 ), x2=( x1 + 2566 ), ans=( x2 + 4 )
 \textbf{Answer}: The answer is 1513.75 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | 2016 | 2015 ( in thousands ) | 2014 |
share-based compensation expense | 30809 | 21056 | 29793 |
income tax benefit | 9879 | 6907 | 7126 |
\\ \colorg & \colorg \textbf{Question}:  how much percent did the income tax benefit increase from 2014 to 2016?
  \\\colorg  & \colorg  \textbf{Rationale:}  x0=( 9879 - 7126 ), ans=( x0 - 7126 )
 \textbf{Answer:} The answer is increased 38.6\%\\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  in billions | 2018 |
january 1 |  33.3 |
issuances | 4.5 |
calls and maturities | -6.8 ( 6.8 ) |
other | -.1 ( .1 ) |
december 31 | 30.9 |
\\\colorg
 &\colorg \textbf{Question}: assuming all matured securities were pledged as collateral , how much should we assume came from the calls?
  \textbf{Rationale:}  ans=( 6.8 - 4.9 ) 
  \textbf{Answer:} The answer is 1.9 \\\cline{2-2}\colorg
    & \colorg\textbf{Table:}  in millions of dollars | u.s . | outside u.s . | december 31 2008 | december 31 2007 |
commercial and similar letters of credit | 2187 | 6028 | 8215 | 9175 |
 \dots\\\colorg
 & \colorg\textbf{Question}: what percentage of citigroup 2019s total other commitments as of december 31 , 2008 are outside the u.s.?
  \textbf{Rationale:}  ans=( 236931 / 1349500 )
  \textbf{Answer:} The answer is 18\%\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\fin{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_fin}
%\vspace{-0.25cm}
\end{table*}
















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: Michael wants to dig a hole 400 feet less deep than twice the depth of the hole that his father dug. The father dug a hole at a rate of 4 feet per hour. If the father took 400 hours to dig his hole \dots ?
\\ & \textbf{Rationale:} Since the father dug a hole with a rate of 4 feet per hour, if the father took 400 hours digging the hole, he dug a hole 4*400 = 1600 feet deep. \dots Michael will have to work for 2800/4 = 700 hours.
\textbf{Answer:} 700
 \\\cline{2-2}
 & \textbf{Question:} When Erick went to the market to sell his fruits, he realized that the price of lemons had risen by $4$ for each lemon. The price of grapes had also increased by half the price that \dots?
 \\ & \textbf{Rationale}:  The new price for each lemon after increasing by $4$ is $8+4 =12$ For the 80 lemons, \dots Erick collected $140*9=1260$ From the sale of all of his fruits, Erick received $1260+960 =2220$.
 \\ & \textbf{Answer}: 2220 \\\cline{2-2}
 & \textbf{Question:}James decides to build a tin house by collecting 500 tins in a week. On the first day, he collects 50 tins. On the second day, he manages to collect 3 times that number. \dots? 
 \\ &\textbf{Rationale:} On the second day, he collected 3 times the number of tins he collected on the first day, which is $3*50 =150$ tins. \dots he'll need to collect $200/4=50$ tins per day to reach his goal. \\&\textbf{Answer:} 50\\\cline{2-2}
  & \textbf{Question:} Darrel is an experienced tracker. He can tell a lot about an animal by the footprints it leaves behind. Based on the impressions, he could tell the animal was traveling east at 15 miles per hour \dots ? \\
 & \textbf{Rationale:} If we let x be the amount of time, in hours, it will take for Darrel to catch up to the coyote, \dots If we subtract 1 x from each side, we get x=1, the amount of time in hours.
 \textbf{Answer:} 1\\\cline{2-2}
    & \textbf{Question:} Martha needs to paint all four walls in her 12 foot by 16 foot kitchen, which has 10 foot high ceilings \dots If Martha can paint 40 square feet per hour, how many hours will it take her to paint kitchen? 
  \\&\textbf{Rationale:} There are two walls that are 12' by 10' and two walls that are 16' by 10' \dots how many hours she needs to finish: 1680 sq ft / 40 sq ft/hour = 42 hours 
  \textbf{Answer:} 42\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The difference between the number of boys and girls in a tree planting event is 400. If there are 600 boys at the event, and the number of girls is more than the number of boys \dots ?
\\ \colorg & \colorg \textbf{Rationale:}  If there are 600 boys at the event, and the difference between boys and girls is 400, there are 600+400=1000 girls.
\dots 60\% of the total number of boys and girls at the event is 60/100*1600=960
\textbf{Answer:} 960
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Casey is trying to decide which employee she wants to hire. One employee works for $\$20$ an hour. The other employee works for $\$22$ an hour, but Casey would also get a $\$6$/hour subsidy \dots ?
\\\colorg  & \colorg\textbf{Rationale}:  First find the weekly cost of the first employee: \$20/hour * 40 hours/week = 800/week \dots subtract the smaller weekly cost from the bigger weekly cost: \$800/week - \$640/week = 160/week.
 \textbf{Answer}: 160 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}Cara has 60 marbles in a bag. 20 of them are yellow, half as many are green, \dots If Cara picks a marble at random, what are the odds it's blue (expressed as a percentage)?
\\ \colorg & \colorg \textbf{Rationale:} First find the number of green marbles: 20 yellow marbles/2=10 green marbles. \dots find the percentage chance of getting a blue marble: 15 marbles/60 marbles*100=25\%.
\textbf{Answer:} 25\\\cline{2-2}\colorg
&\colorg \textbf{Question:} Samir just turned half the age Hania was 10 years ago. If in five years Hania will be 45 years old, what will Samir's age be five years from now?
 \\\colorg  &\colorg 
\textbf{Rationale:} If in five years, Hania will be 45 years old, currently she is 45-5=40 years old. Ten years ago, Hania was 40-10=30 years old. \dots In five years, Samir will be 15+5=20 years old. 
\textbf{Answer:} 20\\\cline{2-2}\colorg
& \colorg\textbf{Question:} If the normal hours of operation of Jean's business are 4 pm to 10p every day Monday through Friday, and from 6 pm to 10 pm on weekends, how many hours is the business open in a week?
\\\colorg
& \colorg \textbf{Rationale:} First, we find the number of hours per weekday by subtracting the smaller number from the larger one \dots We add these two totals together to find that 30+8=38 hours per week.
\textbf{Answer:} 38\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\gsm{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_gsm8k}
%\vspace{-0.25cm}
\end{table*}











\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | Name | Age (years)
| Jessica | 2
| Dalton | 7
| Kelsey | 5
| Lamar | 8
| Alexis | 2
 \textbf{Question}: A girl compared the ages of her cousins. What is the median of the numbers?
\textbf{Rationale:} Read the numbers from the table: 2, 7, 5, 8, 2.
First, arrange the numbers from least to greatest: 2, 2, 5, 7, 8.
Now find the number in the middle. The number in the middle is 5.
The median is 5.
\textbf{Answer: } 5
 \\\cline{2-2}
 & \textbf{Table:} | City | Number of houses sold 
| Melville | 878
| New Hamburg | 871
| Charles Falls | 881
| Pennytown | 817
\textbf{Question}: A real estate agent looked into how many houses were sold in different cities. Where were the fewest houses sold? \textbf{Rationale}: Find the least number in the table. \dots The least number is 817.
Now find the corresponding city. Pennytown corresponds to 817.
   \textbf{Answer}: 817  \\\cline{2-2}
 & \textbf{Table:} | Day | Number of new customers
| Saturday | 2
| Sunday | 2
| Monday | 9
| Tuesday | 4
| Wednesday | 10
| Thursday | 3
| Friday | 6
\textbf{Question}: A cable company analyst paid attention to how many new customers it had each day. What is the median of the numbers?
\textbf{Rationale:} Read the numbers \dots Now find the number in the middle. The number in the middle is 4.
The median is 4.
  \textbf{Answer:} 4 \\\cline{2-2}
  & \textbf{Table:} | Day | Number of cups
| Friday | 8
| Saturday | 4
| Sunday | 10
| Monday | 6
| Tuesday | 6
| Wednesday | 1
| Thursday | 0
 \textbf{Question}: Nancy wrote down how many cups of lemonade she sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 8, 4, 10, 6, 6, 1, 0. \dots Subtract the least number from the greatest number: 10-0=10. The range is 10.
\textbf{Answer:} 10\\\cline{2-2}
    & \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
|\$700 | 9,800 | 22,600
|\$740 | 8,000 | 22,800
|\$780 | 6,200 | 23,000
|\$820 | 4,400 | 23,200
|\$860 | 2,600 | 23,400
\textbf{Question}: At a price of \$860, is there a shortage or a surplus?
 \textbf{Rationale:} At price of \$860, quantity demanded is less than quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
 \textbf{Answer:}  surplus\\
 \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | Day | Number of tickets
| Monday | 36
| Tuesday | 43
| Wednesday | 46
| Thursday | 59
| Friday | 37
| Saturday | 46
| Sunday | 51
\textbf{Question}: The transportation company tracked the number of tickets sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 36, 43, 46, 59, 37, 46, 51. Find greatest number. The greatest number is 59. Find least
number. The least number is 36. Subtract least from the greatest number: 59 - 36 = 23.
The range is 23.
\textbf{Answer: } 23
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | Stem | Leaf 
| 4 | 2, 7, 9, 9, 9
| 5 | 1
| 6 | 9
| 7 | 2, 2, 3, 3, 5
| 8 | 
| 9 | 0
\textbf{Question}:  A pottery factory kept track of the number of broken plates per shipment last week. How many shipments had exactly 73 broken plates?
\textbf{Rationale}:  For the number 73, the stem is 7, and the leaf is 3. Find the row where the stem is 7. In that row, count all the leaves equal to 3.
You counted 2 leaves, which are blue in the stem-and-leaf plot above. 2 shipments had exactly 73 broken plates.
\textbf{Answer}: 2 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | purple and red clay bead | \$0.02
| small pink bead | \$0.04
| pearl bead | \$0.07
| round silver bead | \$0.01
| brown cat's eye bead | \$0.08
| orange glass bead | \$0.07
\textbf{Question}:  Kylie has \$0.05. Does she have enough to buy a small pink bead and a purple and red clay bead?
\textbf{Rationale:}  Add the price of a small pink bead and the price of a purple and red clay bead: \$0.04 + \$0.02 = \$0.06
\$0.06 is more than \$0.05. Kylie does not have enough money.
\textbf{Answer:} Kylie does not have enough money.  \\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
| \$165 | 17,900 | 6,400
| \$345 | 15,100 | 8,900
| \$525 | 12,300 | 11,400
| \$705 | 9,500 | 13,900
| \$885 | 6,700 | 16,400
\textbf{Question}: Look at the table. Then answer the question. At a price of \$885, is there a shortage or a surplus?
\textbf{Rationale:}  At the price of \$885, the quantity demanded is less than the quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
\textbf{Answer:} surplus \\\cline{2-2}\colorg
& \colorg\textbf{Table:} | Chickenville | 3:00 A.M. | 12:00 P.M. | 3:30 P.M.
| Floral Gardens | 3:45 A.M. | 12:45 P.M. | 4:15 P.M.
| Pleasant River Campground | 4:45 A.M. | 1:45 P.M. | 5:15 P.M.
| Happy Cow Farm | 5:15 A.M. | 2:15 P.M. | 5:45 P.M.
| Rocky Ravine Town | 5:45 A.M. | 2:45 P.M. | 6:15 P.M.
\textbf{Question}: Look at the following schedule. Doug just missed the 3.00 A.M. train at Chickenville. How long does he have to wait until the next train?
\textbf{Rationale:}  Find 3:00 A. M. in the row for Chickenville. Look for the next train in that row.
The next train is at 12:00 P. M. The elapsed time is 9 hours.
\textbf{Answer:} 9\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\tab{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_tabmwp}
%\vspace{-0.25cm}
\end{table*}



















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS & \textbf{Facts}: Penguins are native to the deep, very cold parts of the southern hemisphere. Miami is located in the northern hemisphere and has a very warm climate.
 \\&\textbf{Question:} Would it be common to find a penguin in Miami?
\\ & \textbf{Rationale:} Where is a typical penguin's natural habitat? What conditions make \#1 suitable for penguins? Are all of \#2 present in Miami?
\textbf{Answer: No}
 \\\cline{2-2}
 & \textbf{Facts:} Shirley Bassey recorded the song Diamonds are Forever in 1971. Over time, diamonds degrade and turn into graphite. Graphite is the same chemical composition found in pencils.
\\ &\textbf{Question:} Is the title of Shirley Bassey's 1971 diamond song a true statement?
 \textbf{Rationale}: What is the title to Shirley Bassey's 1971 diamond song? Do diamonds last for the period in \#1? \textbf{Answer}: No \\\cline{2-2}
 & \textbf{Facts:} The first six numbers in the Fibonacci sequence are 1,1,2,3,5,8. Since 1 is doubled, there are only five different single digit numbers.  \textbf{Question:} Are there five different single-digit Fibonacci numbers?
 \\ &\textbf{Rationale:} What are the single-digit numbers in the Fibonacci sequence? How many unique numbers are in \#1? Does \#2 equal 5?
\textbf{Answer:} Yes\\\cline{2-2}
  & \textbf{Facts:} Katy Perry's gospel album sold about 200 copies. Katy Perry's most recent pop albums sold over 800,000 copies.
\textbf{Question:} Do most fans follow Katy Perry for gospel music?
 \textbf{Rationale:} What type of music is Katy Perry known for? Is Gospel music the same as \#1?
 \textbf{Answer:} No\\\cline{2-2}
    & \textbf{Facts:} The Italian Renaissance was a period of history from the 13th century to 1600. A theocracy is a type of rule in which religious leaders have power. Friar Girolamo Savonarola was the ruler of Florence, after driving out the Medici family, from November 1494 â€ 23 May 1498. \textbf{Question:} Was Florence a Theocracy during Italian Renaissance?
  \textbf{Rationale:} When was the Italian Renaissance?When did Friar Girolamo Savonarola rule Florence? Is \#2 within the span of \#1? Did Friar Girolamo Savonarola belong to a religious order during \#3?
  \textbf{Answer:} Yes\\
  \midrule




  
\colorg \static{} & \colorg \textbf{Facts}: The average cost of a US Boeing 737 plane is 1.6 million dollars. Wonder Woman (2017 film) grossed over 800 million dollars at the box office. \textbf{Question}: Is a Boeing 737 cost covered by Wonder Woman (2017 film) box office receipts?
 \textbf{Rationale:}  How much does a Boeing 737 cost?. How much did the 2017 movie Wonder Woman gross? Is \#2 greater than \#1?
\textbf{Answer:} Yes
 \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Big Show is a professional wrestler that weighs 383 pounds. Force is equal to mass times acceleration. An adult Cheetah weighs around 160 pounds. An adult Cheetah can run up to 58 MPH. \textbf{Question:}  Can a cheetah generate enough force to topple Big Show?
\colorg\textbf{Rationale}:  How much does Big Show weigh? How much does a cheetah weigh? How fast can a cheetah run? Is the force produced by a mass of \#2 and a speed of \#3 enough to knock over something that weighs \#1?
 \textbf{Answer}: Yes \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Spaghetti and meatballs are a staple on Italian pizzeria menus in the US. The Olive Garden, an Italian family restaurant, has several dishes with meatballs. Meatballs originated in the Chinese Qin dynasty (221 BC to 207 BC). \textbf{Question:} Do restaurants associate meatballs with the wrong country of origin?
 \textbf{Rationale:} In what country is the oldest evidence of people eating meatballs found? What dish involving meatballs became popular in the United States after being invented in New York City in the 20th century? With which national cuisine do Americans typically associate \#2? Are \#3 and \#1 different?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Torah scrolls must be duplicated precisely by a trained scribe. The Torah has a total of 8,674 words. The population of Bunkie Louisiana is 3,939 people according to a 2018 census. \\ \colorg &\colorg \textbf{Question:} Can you give at least one word from the Torah to all residents of Bunkie Louisiana?
\textbf{Rationale:} How many words are in the Torah? How many residents does Bunkie, Louisiana have? Is \#1 greater than \#2?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Wrestlemania X took place in 1994. The Toyota Prius was first manufactured in 1997. \textbf{Question:} Could someone have arrived at Wrestlemania X in a Toyota Prius?
\textbf{Rationale:} When did Wrestlemania X hold? When was the Toyota Prius first manufactured? Is \#2 before \#1?
\textbf{Answer:} No\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\strat{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_strategyqa}
%\vspace{-0.25cm}
\end{table*}

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{purple}
% Is our method specific to in-context numerical reasoning, or can it also work for other NLU tasks? What is special about numerical reasoning? Can we say that we design a general method but test it on numerical reasoning tasks because they are more difficult? \color{green} As semantic similarity between train and test set can't be used to select ICEs in case of numerical reasoning. Therefore we propose EXPLORA.\\
% \color{black}
% \color{blue}
% - We are given only the task-specific loss, which is different from generative model error. We do not utilize the logits given by generative models. Bayesian explanation, in-context one iteration GD -- each of these papers, can we say why these theories don't apply to complex QA.

% Complex numerical reasoning tasks such as financial question answering \cite{chen2022finqa} or tabular question answering \cite{tabmwp} require both language understanding as well as reasoning skills.
% Large language models (LLMs) have been shown to exhibit both these skills.
% Language understanding skills help  While 

% \color{gray}

Answering complex questions that require multi-step numerical reasoning \cite{chen2022finqa,tabmwp,aqua_rat,roy2016solving} over structured and unstructured sources is an active research area with applications in finance, law, and healthcare~\cite{wang2023survey}.
% The complexity in such tasks could arise from multiple factors, such as the need to parse heterogeneous sources like tables and text \cite{chen2022finqa} coupled with multi-step numerical reasoning \cite{tabmwp,aqua_rat,roy2016solving} to answer the question. 

Existing supervised approaches for numerical reasoning involve fine-tuning of multiple generative models for generating arithmetic programs or stepwise solution to the original problem \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa,aqua_rat,roy2016solving,geva-etal-2020-injecting,cobbe2021training}. 
 
% However, existing approaches require expensive annotations of supervised stepwise rationales along with the solution for fine-tuning multiple generative models \cite{aqua_rat} \cite{cobbe2021training} \cite{geva-etal-2020-injecting} lacking a general purpose solution. 

\begin{figure*}[t]
\centering

\includegraphics[width=0.8\textwidth]{figures/explora-cropped.pdf}\\
\caption{Overview of \static{}, proposed exemplar selection approach.}
\label{fig:icl}
% \vspace{-4mm}
\end{figure*}


More recently, the advances in Large Language Models (LLMs) has lead to substantial progress in a wide range of natural language understanding and reasoning tasks \cite{brown2020gpt3}. The emergent capabilities in LLMs\cite{wei2022emergent,gpt3incontext} such as In-Context Learning (ICL) has paved the way to a new class of approaches that employ chain-of-thought reasoning~\cite{complex_cot} \cite{wei2023chainofthought} for solving complex numerical reasoning questions.
Instead of fine-tuning task-specific models, these approaches focus on choosing carefully constructed exemplars with rationales to be used as input to LLMs, commonly termed as prompting.
% A distinct advantage of prompting with demonstration samples vs fine-tuning is  that the LLM is a general-purpose machine that can be used to solve multiple numerical reasoning tasks.
% In this paper, our focus is to propose a general framework that can be employed to solve multiple QA tasks that require numerical reasoning over homogeneous and heterogeneous sources by selecting suitable demonstration samples.

\mpara{The limitations of manual exemplar selection.} 
% It is inherently hard for the LLMs to perform multi-step reasoning using few-shot in-context learning with just the  \texttt{(input, output)} pairs~\cite{rae2022scaling}.
To tackle complex numerical reasoning problems, \textit{chain-of-thought} (COT) prompting was proposed to add hand-crafted natural language rationales (stepwise solutions) to the prompts in addition to input and output resulting in \texttt{(input, rationale, output)}~\cite{wei2023chainofthought}.
% The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort \cite{wei2023chainofthought} \cite{brown2020gpt3}.

% Interesting, 
% COT rationales for compositional natural language questions involve generating explanations for the final answer. 
% However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. 
% In such cases, the decomposition of such question to simpler sub-questions is observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted follow-up questions derived from the original complex questions to the prompt.
However, there are inherent limitations of COT approach for complex and hybrid numerical reasoning tasks. 
The COT involves the manual effort of selecting the best exemplars with appropriate rationales that sufficiently convey the  execution strategy for the task under consideration. The manual selection process is tedious and not scalable across different numerical reasoning tasks. Since the outputs generated by the LLM are highly sensitive to exemplars provided \cite{lu-etal-2022-fantastically,zhao2021calibrate,chang2023data}, it is crucial to select meaningful exemplars that are robust across evaluation samples and improve overall task performance.

\mpara{Limitations of automated exemplar selection approaches}:
To tackle these limitations, several automated exemplar selection approaches have been proposed \cite{ye2023compositional,lu-etal-2022-fantastically,rubin-etal-2022-learning,complex_cot}. These approaches are usually dynamic exemplar selection methods, which select several demonstration examples from the training set for each test example. Several approaches also require annotated data and training of several models for exemplar selection\cite{lu2023dynamic,ye2023compositional}. These approaches entail to heavy computational requirements during inference, especially when there is a large pool of exemplars to select from. While unsupervised approaches like similarity \cite{rubin-etal-2022-learning} or diversity based \cite{ye-etal-2023-complementary} approaches exist for dynamic exemplar selection, they also require projecting the input query and the entire pool of exemplars to a continuous vector space followed by search, increasing computational time during inference. Additionally, the majority of these approaches assume the exemplars chosen to be independent of each other and only consider the interaction between the test sample and the exemplars. They do not account for the interactions between the exemplars themselves.

 As an alternative to dynamic exemplar selection approaches, LENS \cite{li2023finding} proposed to select a static set of task level support exemplars. However, LENS assumes access to language model output logits and involves multiple expensive evaluations of the LLM for scoring the exemplars. LENS also does not model the interactions between exemplars and scores each sample independently. 
% In the example below, using Few-shot-COT results in inaccurate results due to lack of decomposition information in its prompt (hidden due to space reasons).
% \input{intro-example-mouth}

\mpara{\static{} (Static Exemplar Selection Approach):}
In this work, we propose a novel static exemplar selection method \static{}, that selects multiple high value/low loss exemplar subsets. An overview of the working of \static{} is shown in Figure \ref{fig:icl}. The selection of task level exemplar subsets are performed once, and we model the interactions between exemplars through initial sampling of subsets and by directly scoring and selecting subsets. We propose a parameterized scoring function that approximates the loss indicative of task performance using features from a transformer based embedding model. We propose an exploration mechanism as shown in Figure \ref{fig:icl} to estimate the parameters of the scoring function with minimal calls to the LLM and without access to logits from the LLM. Our approach mitigates the expensive processing during inference incurred by traditional dynamic exemplar selection approaches and obviates the need for manual exemplar selection while providing high performance.


\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new robust static exemplar selection approach \static{}, that selects task level exemplars for numerical reasoning based questions.

    \item 
    2) We demonstrate the ability of transferring selected exemplars across models. We show that exemplars selected using smaller models can be used to induce reasoning capabilities in much larger models leading to reduced costs.
     \item 
     3) We demonstrate that \static{} is less resource intensive compared to existing approaches, as it results in minimal calls to the LLMs for exemplar selection.
    \item 
    4) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of \static{} across multiple complex and hybrid numerical reasoning based QA tasks.
\end{description}

\color{black}


==> line-plot.tex <==
\begin{tikzpicture}
\begin{axis}[
    xlabel=Number of LLM calls ($*10^3$),
    ylabel=Exact match,
    xmin=0.8, xmax=2.6,
    ymin=54, ymax=75]
    xtick={50,52,54,56...,75}
\addplot[smooth,mark=*,darkblue] plot coordinates {
    (1,57)
    (1.2,57.5)
    (1.4,59)
    (1.6,61)
    (1.8,63)
    (2.0,64.5)
    (2.2,65.5)
    (2.4,66.5)};
\addlegendentry{\tab{}}

\addplot[smooth,color=red,mark=x]
    plot coordinates {
    (1,65.5)
    (1.2,66)
    (1.4,67)
    (1.6,67.5)
    (1.8,68)
    (2.0,68.5)
    (2.2,69)
    (2.4,69)
    };
\addlegendentry{GSM8K}
\end{axis}
    \end{tikzpicture}
